New Beta Cephei stars with KELT

We present the results of a search for Galactic Beta Cephei stars, which are massive pulsating stars with both pressure modes and mixed modes. Thus, these stars can serve as benchmarks for seismological studies of the interiors of massive stars. We conducted the search by performing a frequency analysis on the optical light curves of known O- and B-type stars with data from the KELT exoplanet survey. We identify 113 Beta Cephei stars, of which 86 are new discoveries, which altogether represents a ~70% increase in the number presently known. An additional 96 candidates are identified. Among our targets, we find five new eclipsing binaries and 22 stars with equal frequency spacings suggestive of rotational splitting of nonradial pulsation modes. Candidates for runaway stars among our targets and a number of interesting individual objects are discussed. Most of the known and newly discovered Beta Cephei stars will be observed by the TESS mission, providing by far the most comprehensive observational data set of massive main sequence pulsating stars of sufficient quality for detailed asteroseismic studies. Future analysis of these light curves has the potential to dramatically increase our understanding of the structure of stellar interiors and the physical processes taking place therein.

==> Tbl_bcepfreq.tex <==
\startlongtable 
\begin{deluxetable}{lcr}  
\tablecaption{Frequencies and amplitudes determined for the \Bcep stars. Formal error estimates determined according to \citet{Montgomery1999} are given in braces in units of the last significant digit. \dag Amplitudes may be largely suppressed.}
\label{tbl:bcep-freqtable}
\tablenum{7}
\tablehead{ 
\colhead{ID} & \colhead{Freq.}    & \colhead{Amp.}\\
\colhead{ } & \colhead{(d$^{-1}$)} & \colhead{(mmag)}
}
\startdata
\hline \multicolumn{3}{c}{TIC 5076425} \\
\hline
F1&	5.63875(1)&37(1) \\
F2&	5.88842(1)&33(1) \\
F3&	5.81121(2)&	20(1) \\
F4&	5.45326(4)&10(1) \\
\hline 
\enddata
\tablecomments{This table is published in its entirety in the machine-readable format. A portion is shown here for guidance regarding its form and content.}
\end{deluxetable}

==> Tbl_candfreq.tex <==
\startlongtable 
\begin{deluxetable}{lcr}  
\tablecaption{Frequencies and amplitudes determined for the Candidate \Bcep stars. Formal error estimates determined according to \citet{Montgomery1999} are given in braces in units of the last significant digit. \dag Amplitudes may be largely suppressed.}
\label{tbl:cand-freqtable}
\tablenum{8}
\tablehead{ 
\colhead{ID} & \colhead{Freq.}    & \colhead{Amp.}\\
\colhead{ } & \colhead{(d$^{-1}$)} & \colhead{(mmag)}
}
\startdata
\hline
\multicolumn{3}{c}{TIC 92193} \\
\hline
F1&	5.97644(5)&1.6(2)\\
\hline 
\multicolumn{3}{c}{TIC 11158867} \\
\hline
F1&	12.91477(8)&2.0(3) \\
F2&	1.54085(9)&1.8(3) \\
\hline 
\enddata
\tablecomments{This table is published in its entirety in the machine-readable format. A portion is shown here for guidance regarding its form and content.}
\end{deluxetable}

==> Tbl_rejfreq.tex <==
\startlongtable 
\begin{deluxetable}{lcr}  
\tablecaption{Frequencies and amplitudes determined for the rejected stars. Formal error estimates determined according to \citet{Montgomery1999} are given in braces in units of the last significant digit.}
\label{tbl:rejected-freqtable}
\tablenum{9}
\tablehead{ 
\colhead{ID} & \colhead{Freq.}    & \colhead{Amp.}\\
\colhead{ } & \colhead{(d$^{-1}$)} & \colhead{(mmag)}
}
\startdata
\hline 
\multicolumn{3}{c}{TIC 12647620} \\ %initially a cand
\hline
F1&	3.51173(5)&4.8(4) \\
F2&	1.24177(8)&3.0(4) \\
\hline \multicolumn{3}{c}{TIC 26283875} \\ \hline
F1&	14.24270(9)&0.8(1) \\ 
\hline
\enddata
\tablecomments{This table is published in its entirety in the machine-readable format. A portion is shown here for guidance regarding its form and content.}
\end{deluxetable}
